Impact of AI Search Summaries on Website Traffic: Evidence from Google AI Overviews and Wikipedia

Search engines increasingly display AI-generated answers above organic links, potentially displacing traffic to upstream publishers. We estimate the impact of Google's AI Overviews (AIO) on Wikipedia's search traffic using AIO's staggered geographic rollout and Wikipedia's multilingual structure. Our difference-in-differences design compares monthly external-search referrals to English Wikipedia articles with referrals to the same articles in German and French, and finds that default AIO availability reduced English search traffic by 5.45% and 4.82%, respectively. Our results suggest that answer-producing digital intermediaries can materially reallocate attention away from informational publishers, with implications for content monetization, search platform design, and policy.

==> figures/clickstream/unfiltered/event_studies.tex <==
\begin{figure}[htp!]
\centering
\begingroup
\small
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}>{\centering\arraybackslash}m{0.325\textwidth}>{\centering\arraybackslash}m{0.325\textwidth}>{\centering\arraybackslash}m{0.325\textwidth}@{}}
English--Japanese & English--German & English--French \\
\paperassetgraphic[width=\linewidth,keepaspectratio]{figures/clickstream/unfiltered/event_study_ja.pdf} & \paperassetgraphic[width=\linewidth,keepaspectratio]{figures/clickstream/unfiltered/event_study_de.pdf} & \paperassetgraphic[width=\linewidth,keepaspectratio]{figures/clickstream/unfiltered/event_study_fr.pdf} \\
\end{tabular}
\endgroup
\caption{Monthly PPML event-study estimates for the pair-specific full-coverage samples. March 2024 is the omitted reference month and April 2024 is event month zero. Pointwise 95\% confidence intervals use two-way-clustered standard errors.}
\label{fig:clickstream_unfiltered_event_studies}
\end{figure}


==> figures/clickstream/unfiltered/honestdid_rm.tex <==
\begin{figure}[htp!]
\centering
\begingroup
\small
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}>{\centering\arraybackslash}m{0.325\textwidth}>{\centering\arraybackslash}m{0.325\textwidth}>{\centering\arraybackslash}m{0.325\textwidth}@{}}
English--Japanese & English--German & English--French \\
\paperassetgraphic[width=\linewidth,keepaspectratio]{figures/clickstream/unfiltered/honestdid_rm_ja.pdf} & \paperassetgraphic[width=\linewidth,keepaspectratio]{figures/clickstream/unfiltered/honestdid_rm_de.pdf} & \paperassetgraphic[width=\linewidth,keepaspectratio]{figures/clickstream/unfiltered/honestdid_rm_fr.pdf} \\
\end{tabular}
\endgroup
\caption{Honest DiD sensitivity intervals under relative-magnitude ($\Delta^{RM}$) restrictions for Japanese, German, and French controls. The target is the equally weighted average of April--December 2024, using the original full PPML event-study covariance matrices.}
\label{fig:clickstream_unfiltered_honestdid_rm}
\end{figure}


==> figures/clickstream/unfiltered/log_referrals.tex <==
\begin{figure}[htp!]
\centering
\begingroup
\small
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}>{\centering\arraybackslash}m{0.325\textwidth}>{\centering\arraybackslash}m{0.325\textwidth}>{\centering\arraybackslash}m{0.325\textwidth}@{}}
English--Japanese & English--German & English--French \\
\paperassetgraphic[width=\linewidth,keepaspectratio]{figures/clickstream/unfiltered/model_free_ja.png} & \paperassetgraphic[width=\linewidth,keepaspectratio]{figures/clickstream/unfiltered/model_free_de.png} & \paperassetgraphic[width=\linewidth,keepaspectratio]{figures/clickstream/unfiltered/model_free_fr.png} \\
\end{tabular}
\endgroup
\caption{Demeaned log total monthly search traffic in the pair-specific full-coverage samples. Each English and control series is demeaned using November 2023--March 2024; the dashed line marks April 2024.}
\label{fig:clickstream_unfiltered_log_referrals}
\end{figure}

